Analysis of structured Markov processes

Markov processes are popular mathematical models, studied by theoreticians for their intriguing properties, and applied by practitioners for their flexible structure. With this book we teach how to model and analyze Markov processes. We classify Markov processes based on their structural properties, which in turn determine which analytic methods are required for solving them. In doing so, we start in each chapter with specific examples that naturally lead up to general theory and general methods. In this way the reader learns about Markov processes on the job. By studying this book, the reader becomes acquainted with the basic analytic methods that come into play when systems are modeled as structured Markov processes. These basic methods will likely prove useful, in real-time when studying the examples at hand, but more importantly for future encounters with Markov processes not covered in this book. Methods are more important than examples. The methods have a large scope of application, even outside the scope of Markov processes, in areas like probability theory, industrial engineering, mechanical engineering, physics and financial mathematics.

==> SupportFiles/tikz_settings.tex <==
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat = newest}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{calc}

% Introduce an additional layer
\pgfdeclarelayer{arrowlayer}
\pgfsetlayers{main,arrowlayer}

% Define some `newcommands' for tikz usage
\tikzset{%
    > = {Latex[width=1.7mm,length=2.2mm]}%
    }%

\tikzset{%
    state/.style = {%
        draw, circle, minimum size = 4, inner sep = 0, fill = black
    }%
}%

\tikzset{%
    statelarge/.style = {%
        draw, circle, minimum size = 15pt, inner sep = 0pt
    }%
}%

\tikzset{%
    dashedarrow/.style = {%
        draw, densely dashed, > = {Latex[width = 1.7mm, length = 2.2mm, open, fill = white]}, decoration = {markings, mark = at position 0.999 with {\begin{pgfonlayer}{arrowlayer} \arrow{>} \end{pgfonlayer}}},
        postaction = {decorate}
    }%
}% 
